The Role of Valence and Meta-awareness in Mirror Self-recognition Using Hierarchical Active Inference

The underlying processes that enable self-perception are crucial for understanding multisensory integration, body perception and action, and the development of the self. Previous computational models have overlooked an essential aspect: affective or emotional components cannot be uncoupled from the self-recognition process. Hence, here we propose a computational approach to study self-recognition that incorporates affect using state-of-the-art hierarchical active inference. We evaluated our model in a synthetic experiment inspired by the mirror self-recognition test, a benchmark for evaluating self-recognition in animals and humans alike. Results show that i) negative valence arises when the agent recognizes itself and learns something unexpected about its internal states. Furthermore, ii) the agent in the presence of strong prior expectations of a negative affective state will avoid the mirror altogether in anticipation of an undesired learning process. Both results are in line with current literature on human self-recognition.

==> abstract.tex <==



==> conclusions.tex <==
\chapter{Conclusions}\label{conclusions}
In this chapter you present all conclusions that can be drawn from the preceding chapters.
It should not introduce any new material or theories, these should have been written down earlier in the thesis. Because of this, your conclusion can be brief and to the point.




